Computational Grounding of Responsibility Attribution and Anticipation in LTLf

Responsibility is one of the key notions in machine ethics and in the area of autonomous systems. It is a multi-faceted notion involving counterfactual reasoning about actions and strategies. In this paper, we study different variants of responsibility in a strategic setting based on LTLf. We show a connection with notions in reactive synthesis, including synthesis of winning, dominant, and best-effort strategies. This connection provides the building blocks for a computational grounding of responsibility including complexity characterizations and sound, complete, and optimal algorithms for attributing and anticipating responsibility.

==> sections/reproducibility-checklist.tex <==
\newpage
\section*{Reproducibility Checklist}

This paper:

\begin{itemize}
   \item Includes a conceptual outline and/or pseudocode description of AI methods introduced:
       \textbf{YES}
   \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results:
       \textbf{YES}
   \item Provides well-marked pedagogical references for less-familiar readers to gain the background necessary to replicate the paper:
       \textbf{YES}
\end{itemize}

Does this paper make theoretical contributions? 
\textbf{YES}\\

If yes, please complete the list below.

\begin{itemize}
   \item All assumptions and restrictions are stated clearly and formally.
       \textbf{YES.}
   \item All novel claims are stated formally (e.g., in theorem statements).
       \textbf{YES.}
   \item Proofs of all novel claims are included.\\
       \textbf{YES.} It is in the supplementary material.
   \item Proof sketches or intuitions are given for complex and/or novel results.
       \textbf{YES.}
   \item Appropriate citations to theoretical tools used are given.
       \textbf{YES.}
   \item All theoretical claims are demonstrated empirically to hold.
       \textbf{N.A.}
   \item All experimental code used to eliminate or disprove claims is included.
       \textbf{N.A.}
\end{itemize}

Does this paper rely on one or more datasets?
\textbf{NO.}\\

Does this paper include computational experiments?
\textbf{NO.}\\
